Automated Conversion of Music Videos into Lyric Videos

Musicians and fans often produce lyric videos, a form of music videos that showcase the song's lyrics, for their favorite songs. However, making such videos can be challenging and time-consuming as the lyrics need to be added in synchrony and visual harmony with the video. Informed by prior work and close examination of existing lyric videos, we propose a set of design guidelines to help creators make such videos. Our guidelines ensure the readability of the lyric text while maintaining a unified focus of attention. We instantiate these guidelines in a fully automated pipeline that converts an input music video into a lyric video. We demonstrate the robustness of our pipeline by generating lyric videos from a diverse range of input sources. A user study shows that lyric videos generated by our pipeline are effective in maintaining text readability and unifying the focus of attention.

==> abstract.tex <==
\begin{abstract}
% problem
Musicians and fans often produce lyric videos, a form of music videos that showcase the song's lyrics, for their favorite songs.
However, making such videos can be challenging and time-consuming as the lyrics need to be added in synchrony and visual harmony with the video.
% contribution, mention overall goals?
Informed by prior work and close examination of existing lyric videos, we propose a set of design guidelines to help creators make such videos.
Our guidelines ensure the readability of the lyric text while maintaining a unified focus of attention.
We instantiate these guidelines in a fully automated pipeline that converts an input music video into a lyric video.
% The user can further edit the output videos for more stylized and artistic expressions.
% results and evaluation
We demonstrate the robustness of our pipeline by generating lyric videos from a diverse range of input sources.
A user study shows that lyric videos generated by our pipeline are effective in maintaining text readability and unifying the focus of attention.

% Texts, such as captions, subtitles, quotes, and labels, are essential to make videos more accessible, understandable, and enjoyable to a wide range of audiences.
% %
% However, current video subtitles use texts only as literal transcriptions of speeches, omitting all the other linguistic and paralinguistic information such as tone, pitch, and emotion.
% %
% In addition to their literal content, texts can capture the richness of spoken words by dynamically changing their forms to express emotion, portray characters, direct attention, and visualize sound and motion.
% Such dynamic texts, more often referred to as \textit{kinetic typography}, have found a wide range of applications in design, animation, and video post-processing.
% One important application is the use of dynamic texts to enhance captions or create text effects in videos to convey the underlying mood and emotions of the speakers and narrations or the underlying artistic feels of sound effects in noisy environments and for deaf or hard of hearing (DHH) people~\cite{Hersh:2013:DPE}.
% However, there is a lack of authoring guidelines and tools for ordinary users to create such dynamic textual effects efficiently and effectively for videos.

% We propose {\em embodied kinetic typography}, a new type of stylized, animated texts that can dynamically change their appearances and interact with the video content like speech, music, sound, and mood.
%
% Similar to works like embodied graphics~\cite{Saquib:2019:IBD} and algebra~\cite{Saquib:2021:CEA}, we propose a system that can help ordinary users create such embodied kinetic typography with their video content, inspired by fundamental issues in graphics, HCI, accessibility, and human perception (embodied cognition).
%
% In our work, we explored how kinetic typography can be used to enhance the video subtitle experience, and contribute:
% 1) a design framework that guides the creation of subtitles that convey the underlying video content with desired kinetic typography effects,
% and
% 2) a text-based authoring tool that allows novice users to create such augmented subtitles via bi-directional direct manipulation without requiring more complex user interfaces and interactions,
% 3) a set of examples made by our tool that demonstrate its robustness and usability, with a focus on talking-head videos.
%automatically adds embodied kinetic typography as captions to videos while allowing users to predefine and customize certain behaviors.
% We conduct a user study to validate whether our proposed system can help the creation of animated texts to convey stylized, expressive, emotional, and visual information, as well as enhance memorability and appeal with or without the video sound.

\end{abstract}


==> background.tex <==
\section{Background}
% Lyrics added to videos are similar in function as video subtitles, and it is essential to ensure that subtitles are easy to read. \maneesh{Point about readability should come earlier in the paper -- section on guidelines could come before related work. Then related work can just focus on talking about the related papers.}
%
% \maneesh{Prev. sentence is about the design guidelines, not about related work. should move there. In fact this entire section is likely better in the design guidelines section.}

% \subsection{Terminology}

% \paragraph{Lyric flash}
% In subtitling, a {\em subtitle flash} means ``an individual, uninterrupted one- or two-line subtitle text that appears on the screen between specific in and out times''~\cite{Perego:2008:WWW}.
% We hence use the term \textit{lyric flash} to refer to the equivalent of subtitle flash in the context of lyric videos.

% \paragraph{Vision span}
Fundamentally, human eyes can see objects within the field of vision but can only read text in a narrow angular vision span of $6^{\circ}$ vertically and horizontally~\cite{}. 
Figuratively, this means that the viewer can read text within a circular region of $5.23$\,cm in diameter when the screen is $50$\,cm away.
%
This narrow vision span means that if contents of interests are wide or far apart, such as a wide line of text or lyric text placed far away from the video's salient region, the eye gaze needs to move a lot in order to read and comprehend these contents. 
Such extensive movements can lead to eyestrain, negatively affect the readability of the textual contents, and distract the viewer from understanding both the text and the video~\cite{}.
Minimizing the amount of eye movements thus is one of the top priorities in our design guidelines.

% Together, they form the four categories of readability factors for lyric text in videos. Our proposed design guidelines are based on these categories. We explain what each category entails below.

% \paragraph{Text content and layout}
% %
% This category then concerns with which textual segment of the lyrics should be the content of a lyric flash and how the content should be laid out in terms of line breaking.
% \paragraph{Temporal text placement} Temporal placement considers aligning a lyric flash to specific in and out times in the video timeline.
% \paragraph{Spatial text placement} Spatial placement considers where in relation to the video content a lyric flash should be placed. 
% \paragraph{Text animation} Text animation here refers to specific subcategories of animations applied to a lyric flash or individual words in a lyric flash for the purpose of enhancing the readability.\\

% However, human eyes have a limited vision span and can only read texts that lie within that narrow span~\cite{}.
% \liyi{(March 20, 2023) What is "span" here? Do you mean field of view?}%liyi
% The conventional location of subtitles then requires the viewers to constantly move their eye gaze between the subtitle text and the focus of attention of the video imagery. This can negatively affect the readability of the subtitles and lead to eyestrain. 

% Current conventions put subtitles at the bottom of the video frame. 
% \maneesh{I don't think we need to compare to "subtitles". Those have been developed to handle all kinds of video. We are aiming to produce lyrics videos, not videos with subtitles.}

% \maneesh{I don't think it makes sense to compare to subtitles. We should motivate what we do. We don't need to explain the promblems with subtitles. Also note that some systems can place subtitles at the top or bottom of the video frame.}

% \input{math}

==> ccs.tex <==
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%

\begin{CCSXML}
    <ccs2012>
    <concept>
    <concept_id>10003120.10003121</concept_id>
    <concept_desc>Human-centered computing~Human computer interaction (HCI)</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    % <concept>
    % <concept_id>10010405.10010469.10010475</concept_id>
    % <concept_desc>Applied computing~Sound and music computing</concept_desc>
    % <concept_significance>500</concept_significance>
    % </concept>
    % <concept>
    % <concept_id>10010147.10010178.10010224.10010245.10010250</concept_id>
    % <concept_desc>Computing methodologies~Object detection</concept_desc>
    % <concept_significance>100</concept_significance>
    % </concept>
    % <concept>
    % <concept_id>10010147.10010178.10010179.10010183</concept_id>
    % <concept_desc>Computing methodologies~Speech recognition</concept_desc>
    % <concept_significance>100</concept_significance>
    % </concept>
    </ccs2012>
\end{CCSXML}
    
\ccsdesc[500]{Human-centered computing~Human computer interaction (HCI)}
% \ccsdesc[500]{Applied computing~Sound and music computing}
% \ccsdesc[100]{Computing methodologies~Object detection}
% \ccsdesc[100]{Computing methodologies~Speech recognition}
    

\keywords{Design guidelines; video generation; lyrics}


==> copyright.tex <==
\setcopyright{acmlicensed}



==> dart_throw_alg.tex <==
\begin{algorithm}
  \begin{algorithmic}[1]
    \REQUIRE sample domain $\domainsym$ with distance $\dist$ and conflict $\conflictdist$ measure
    \ENSURE output sample set $\sampleset$
    \STATE $\sampleset \assign \emptyset$
    \STATE $\failure \assign 0$ \pcomment{failure count}
    \WHILE{$\domainsym$ is not fully covered and $\failure$ not too high}
    \STATE $\sample \assign \funct{RandomSample}(\domainsym)$
    \IF{$\dist(\sample, \sampleprime) < \conflictdist(\sample, \sampleprime) \; \forall \sampleprime \in \sampleset$}
    \STATE $\sampleset \assign \sampleset \union \sample$ \pcomment{accept trial sample}
    \STATE $\failure \assign 0$
    \ELSE
    \STATE $\failure \assign \failure + 1$
    \ENDIF
    \ENDWHILE
    \RETURN{} $\sampleset$
  \end{algorithmic}
  \Caption{Dart throwing.}
  {%
This is an example of pseudo-code.
  }
  \label{alg:dart_throw}
\end{algorithm}




==> fig_saliency_error.tex <==
\begin{figure}[h]
    \centering
    % \subfloat[Input Frame]{
    \includegraphics[width=0.49\linewidth]{counting_shot_06_00}
        % \label{fig:variety:kor:1}
    % }
    % \subfloat[Output Saliency Map]{
    \includegraphics[width=0.49\linewidth]{counting_shot_06_sal}
        % \label{fig:variety:kor:2}
    % }
    \caption{Saliency detection models can find salient objects that are irrelevant in the context of music videos.}
    % {%
    % }
    \label{fig:saliency_error}
\end{figure}


==> fig_teaser.tex <==
%\begin{figure}[htb]
\begin{teaserfigure}
  \centering
  \includegraphics[width=\textwidth]{figs/raster/fig_teaser}
 \caption
 {
  We propose a set of design guidelines for adding lyrics to music videos in a manner that ensures text readability and unifies the viewer's focus of attention.
  We further implement a fully automated pipeline that instantiates these guidelines to convert an input music video into a lyric video.
  %
  The results shown above demonstrate that our pipeline is able to generate lyric videos from a wide variety of inputs.
  %
  \camready{%
  \emph{%
  Video source: 
  (a) Selfish Soul by Sudan Archives~\cite{Sudan:2022:SS}, 
  (b) August by Taylor Swift \textcopyright Taylor Swift~\cite{swift:2021:A},
  (c) The Scientist by Coldplay~\cite{Coldplay:2022:ts}, 
  (d) Let It Go by Idina Menzel \textcopyright 2013 Hollywood Records, Inc.~\cite{Menzel:2013:LIG},
  (e) iPad by Chainsmokers~\cite{Chainsmokers:2022:I}, 
  (f) Sandman by Ed Sheeran~\cite{Sheeran:2022:S}}.
  }
  % \maneesh{I don't think the input video is providing much. I would remove it and instead mention that the input video is the same as the output without the text in the caption. Also I would reduce to three frames so we can better read the text as those lyrics are important for this paper. Every example should provide a reference to the URL of the input video and say the name of the artist and song.}
  (a, b, d, e) are in landscape format while (c, f) are in portrait format.
  %\liyi{(April 5, 2023) Minor: Not sure if it is an intentional design to have the right-most column very narrow (are those originally portrait videos?), but normally people would expect to see 3 columns of video frames in the same sizes/proportions.}
 }
 \label{fig:teaser}
%\end{figure}
\end{teaserfigure}


==> fig_variety_shows.tex <==
\begin{figure*}[htb]
    \centering
    \subfloat[Captions to show sound effects]{
        \includegraphics[width=0.49\linewidth]{fig_kor_show_1}
        \label{fig:variety:kor:1}
    }
    \subfloat[Captions to describe actions]{
        \includegraphics[width=0.49\linewidth]{fig_kor_show_2}
        \label{fig:variety:kor:2}
    }
    \\
    \subfloat[Captions to emphasize on the current question]{
        \includegraphics[width=0.49\linewidth]{fig_jap_show}
        \label{fig:variety:jap}
    }
    \subfloat[Captions to describe mental state of a character]{
        \includegraphics[width=0.49\linewidth]{fig_chn_show}
        \label{fig:variety:chn}
    }
    \Caption{East Asian variety shows.}
    {%
    }
    \label{fig:variety_shows}
\end{figure*}


==> graphicspath.tex <==
% \graphicspath{
% {figs/vector/}
% {figs/raster/}
% }%graphicspath


==> interface.tex <==
\section{User Interface}
\label{sec:interface}

Congruence Principle:
for effective visual communication, the content and format of the graphics should correspond to the content and format of the concepts to be conveyed \cite{Tversky:2002:ACF}


==> macros.tex <==
%\citestyle{acmauthoryear}
\setcitestyle{square}
\def\textrightarrow{$\rightarrow$}

%% the following commands are plagiarized from Ravi
\newcommand{\pcline }{\rule{0in}{0.0in}    }  % Spacing for pseudo-code.
\newcommand{\pctab  }{\hspace{0.10in}      }  % Pseudo-code indentation.
\newcommand{\pcbigtab  }{\hspace{1.75in}    }  % Pseudo-code indentation.
\newcommand{\pcasgn }{\mbox{$\leftarrow$}  }  % Pseudo-code assignment operator
%%\newcommand{\pcgreater}{\mbox{$\leftarrow$} } % Pseudo-code bigger operator
\newcommand{\pcomment}[1]{\mbox{// {\it #1}}}  % Pseudo-code comments.
\newcommand{\pckeyword}[1]{\mbox{{\bf #1}}}  % Pseudo-code keywords.
\newcommand{\pcspace}{\hspace{0.10in}}

\newcommand{\pcode}[1]{
    \footnotesize
    \vspace{-0.1in}
    \begin{minipage}{100in} % The width argument will be ignored:
                            % See lamport p. 99
    \begin{tabbing} \hspace{0.10in} \= \pctab \= \pctab \= \pctab \= \pcbigtab \= \\
        #1
    \end{tabbing}
    \end{minipage}
%    \vspace{0.15in}
    }
%% enf of the pseudo code environment

\newcommand{\tabtextsize}{\small}
\newcommand{\figtext}[1]{{\footnotesize #1}}

\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}
\newcommand{\Caption}[2]{\caption[#1]{{\em #1} #2}}
\let\oldcaption\caption
\renewcommand{\caption}[2][]{\oldcaption[#1]{{\em #1} #2}}

\newcommand{\invisible}[1]{{\color{white} #1}}
\newcommand{\emacsquote}[1]{{``#1''}}

\definecolor{SithColor}{rgb}{0.7,0,0} % color for Sith
\newcommand{\liyi}[1]{{\color{SithColor} Li-Yi: #1 $\qed$}}
\definecolor{ConsularColor}{rgb}{0,0.4,0} % color for the Jedi Consulars (e.g. Yoda)
\definecolor{GuardianColor}{rgb}{0,0,0.8} % color for the Jedi Guardians (e.g. Obiwan)
\newcommand{\jiaju}[1]{{\color{GuardianColor} Jiaju: #1 $\qed$}}
\newcommand{\vshin}[1]{{\color{ConsularColor} Jeanette: #1 $\qed$}} % Valentina Shin
\newcommand{\jonelson}[1]{{\color{ConsularColor} Erin: #1 $\qed$}} % John Nelson
\newcommand{\rubaiat}[1]{{\color{ConsularColor} Rubaiat: #1 $\qed$}} % Rubaiat Habib
\newcommand{\maneesh}[1]{{\color{red} MA: #1}} % Maneesh Agrawala
\newcommand{\anyi}[1]{{\color{orange} AR: #1}} % Anyi Rao
\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\todo}[1]{\warning{#1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}
\newcommand{\passthrough}[1]{#1}
\newcommand{\replace}[2]{#2} % replace #1 by #2
\newcommand{\camready}[1]{{\color{GuardianColor}#1}}
\renewcommand{\camready}[1]{{#1}}


\definecolor{AudioColor}{rgb}{0.56,0.34,0.62}
\newcommand{\audio}[1]{{\color{AudioColor} Audio: #1}}

\definecolor{NewColor}{rgb}{0.9,0.4,0}
\newcommand{\new}[1]{{\color{NewColor} #1}}
\definecolor{DeleteColor}{rgb}{0.1,0.6,1.0}
\newcommand{\delete}[1]{{\color{DeleteColor} #1}}
\definecolor{MoveColor}{rgb}{0.5,0.1,0.5}
\newcommand{\update}[1]{{\color{MoveColor} #1}}
\renewcommand{\replace}[2]{\delete{#1}\new{#2}}

\newcommand{\psdraftboxDefault}{\psnodraftbox}

\definecolor{figred}{rgb}{1,0,0}
\definecolor{figgreen}{rgb}{0,0.6,0}
\definecolor{figblue}{rgb}{0,0,1}
\definecolor{figpink}{rgb}{1,0.63,0.63}

\ifthenelse{\isundefined{\hili}}
{
\renewcommand{\new}[1]{{#1}}
\renewcommand{\delete}[1]{}
\renewcommand{\update}[1]{{#1}}
}
{
\ifthenelse{\equal{\hili}{0}}
{
\renewcommand{\new}[1]{{#1}}
\renewcommand{\delete}[1]{}
\renewcommand{\update}[1]{{#1}}
}
{}
}

%\renewcommand{\warning}[1]{}

\ifthenelse{\equal{\final}{1}}
{
\renewcommand{\liyi}[1]{}
\renewcommand{\jiaju}[1]{}
\renewcommand{\rubaiat}[1]{}
\renewcommand{\vshin}[1]{}
\renewcommand{\jonelson}[1]{}
\renewcommand{\maneesh}[1]{}
\renewcommand{\anyi}[1]{}

\renewcommand{\warning}[1]{}
\renewcommand{\note}[1]{}

% \renewcommand{\camready}[1]{}
}

\newcommand{\pseudocode}{Algorithm}
\floatstyle{plain}
\newfloat{algorithm}{tbhp}{lop}
\floatname{algorithm}{\pseudocode}

\newcommand{\funct}[1]{\texttt{#1}}

\newcommand{\filename}[1]{\url{#1}}
\newcommand{\foldername}[1]{\url{#1}}

\let\oldparagraph\paragraph
\iffalse
\newcommand{\passage}[1]{\oldparagraph{\textbf{#1}}}
\renewcommand{\paragraph}[1]{\oldparagraph{\textbf{#1}.}} % \liyi{keep/remove that end period depending on whether you want a paragraph title to end with a period}
\else
% \liyi{no boldface from Spencer}
\newcommand{\passage}[1]{\oldparagraph{{#1}}}
\renewcommand{\paragraph}[1]{\oldparagraph{{#1}.}}
\fi

\newcommand{\command}[1]{{\color{black}{\tt #1}}}

\ifdefined\email
\else
\newcommand{\email}[1]{\url{#1}}
\fi

\if@twocolumn
\newcommand{\twocol}{1}
\fi

\newcommand{\myparam}[1]{\textit{\textbf{#1}}}
\newcommand{\mystyle}[1]{\textit{#1}} % to style the name of the preset stylizations (like \mystyle{anticipation})


==> math.tex <==
\subsection{Math Notion}
\anyi{WIP}
Given a music video $\cV$ aligned with its lyrics subtitle $\cL=[l_1, l_2, \cdots, l_m]$. 
where each $l_m$ corresponds to a visual clip $[f_m^{sta}, \cdots ,f_m^{end}]$. $\cV$ can be written as a list of clip,
$$\cV = [ [f_1^{sta}, \cdots ,f_1^{end}], \cdots, [f_m^{sta}, \cdots ,f_m^{end}]].$$

For each clip, we compute the segmentation mask $[s_m^{sta}, \cdots ,s_m^{end}]$ for each frame and apply an average on it $\bar{s}_m$
\anyi{You may define different constraints here}
And these ensemble as the cost map $\bar{c}_m$.
To have a smooth result within one clip, 
we put text, which is represented by a box $(x,y, w,h)$ in the frame with the center point as $x,y$ and width $w$ and height $h$ in one region along this clip.
$$(x,y,w,h) = \text{argmin}T( (x,y, w,h), \bar{c}_m),$$ 
where $T$ computes the overlap between the text box and the cost map.




==> note.tex <==
\section{Blog}

\begin{description}
\input{note_2023}
\input{note_2022}
\input{note_2021}
\end{description}


==> note_2021.tex <==
\item[December 22, 2021]
{
\rubaiat{
couple of high-level questions to ponder.
\begin{enumerate}
\item
what is the design space of kinectic typography in a live (or post) settings?

\item
what are the goals of it (eg, stylization, memorability, engagement, accessiblity)?

\item
how to design authoring tools?
\end{enumerate}
}%rubaiat
}
\item[December 15, 2021]
{
\rubaiat{
Jiaju, another project direction could be leveraging “kinetic typography” (stylized, expressive, emotional, visual) for live transcript visualization. if done well, there are plenty of implicit benefits (other than cool, expressive visualizations) - memorability, accessiblity etc.
}%rubaiat

\jiaju{
Oh I like this idea! A lot of lessons from our animation tool applies here (stylized visuals). The example that immediately comes to my mind are comic captions (see below). I guess we could also use some NLP here to detect semantics, which can determine the visual style. I definitely see a huge gap here as most accessibility research treats captions as pure text, but visual ones can definitely add to memorability and communicate more information than pure texts (emotions, hierarchy, etc). Plus there could be opportunities to make it interactive! I feel like this could be a good direction that merges all of our previous ideas.
}%jiaju

\liyi{
Rubaiat and I briefly chatted about this, and I think it can be a good project in terms of research novelty (HCI and human perception) and applications (both art and accessibility; imagine now deaf people can  "see" the emotion behind speech tones in movies).
}%liyi
}


==> note_2022.tex <==
\item[November 8, 2022]
{
\liyi{
Maneesh commented during today's meeting that his main concern for the project right now is unclear research contribution.
There are many existing works in the realm of using video content to drive synthetic graphical effects, such as those from Rubaiat, Dan Goldman, and Adobe.
There are also related commercial products.
We can add these to \Cref{sec:prior} and use writing as a way to think through the project position, novelty, and contributions. 
}
}
\item[September 26, 2022]
{
\liyi{
Focus on typography only which would require establishing novelty over \cite{Kato:2015:TLI}, or also consider presenter gestures/postures?
}
}
\item[May 24, 2022: HCI seminar presentation]
{
\vshin{
It would be nice if we can also edit the position of the text within the screen by positioning in the document. For example, we can add a little “outline” around each paragraph that is proportional to the screen, and we can move the text around (by adding spaces or tabs).
}%vshin

\liyi{
I can imagine an interface like object-oriented drawing \cite{Xia:2016:OOD} in which the user clicks/selects a region of text on the direct manipulation UI and brings out a contextual menu for additional effects, such as emotion type.
Bidirectional manipulation (as Cuong asked about) can also be a good feature.
}%liyi
}
\item[May 19, 2022]
{
\liyi{
Quick meeting notes (before I forgot); feel free to add/comment:
\begin{itemize}

\item
Direct manipulation UI (without involving additional stuff like time-line, graphs, etc.) can be a very intuitive authoring paradigm, with potential aids from templates/presets, default suggestions (based on speech analysis). What would be the scope/limitation of such direct manipulation?
(I think "context-free" effects that apply to individual words would be excellent for direction manipulation, but less sure about effects that involve multiple parts of the texts.)

\item
Different text effects (including emojis), potential integration with OnAir/Fusion3D?

\item
Automatic detection of important words/sentences/moments

\item
Automatic layout (e.g., line breaks based on the video content and format)?

\item
Applications (avoid too focused on accessibility and try to be about general effects)
\end{itemize}
}%liyi
}
\item[May 3, 2022]
{
\jiaju{
Thanks so much for the brainstorm session today! Here are some notes
\begin{itemize}

\item
First demo, similar to the example above, not emphasizing every word

\item
Short talking head videos (e.g. adobe Sneaks recorded presentations) then generalize to other types

\item
After Effects text presets \cite{MotionIsland:2016:ATA}

\item
https://www.pinterest.ca/pin/431993789265821520/

\item
Find NHL Playoff ads

\item
Try to talk to people who created those Master class videos, or other artists

\item
Audio-visual podcast - visualize podcast

\item
Designing Programmes \cite{Svilen:2017:DP}
\end{itemize}
}%jiaju

\liyi{
Designing Programmes \cite{Gerstner:1964:DP} has a very interesting perspective about themes and variations, as well as modularity/compositionality, both can be part of our design guidelines.
}%liyi

\liyi{
Based on the materials we have gathered so far, it appears to me that we can start by focusing on the meaning of texts (semantics) as the input driver to design our mapping for output effects. The semantics should have broad enough for different applications and yet narrow enough for us to develop a research project, and I will keep an eye open about whether our mapping designs can be generalized to other types of inputs (e.g., music, tone, motion, etc.)

For applications, one possible scoping is "visualizing a few texts at one time" such as short videos, captions, teleprompters, so that we won't have to worry about traditional typography for readability of a lot of texts.
Thoughts are welcome!
}%liyi

}
\item[April 21, 2022]
{
\jiaju{
Hi everyone! Thanks for coming to our meeting today. Again this week's updates can be found \href{https://docs.google.com/presentation/d/1BZAF33mwhLZL3ZecspYON8FKt6ksPxl19wRiFOjcuKY/}{here}.

Meeting notes:
\begin{itemize}
\item
Jiaju to talk to more people about the tech stack (potentially Python and JavaScript)
\item
Rubaiat to organize a brainstorming session to look at existing examples and application scenarios
\end{itemize}
}%jiaju

\liyi{
Design of the interface and interaction scenarios would guide our methods and implementation, so very important.

Method: on a higher level, we need a font animation engine, which includes morphing/interpolation as a subset.

Implementation: js/html is popular for designers (e.g., web) while python for machine learning researchers (e.g., font interpolation in latent space). On this, I should mention that Zhaowen has done a lot of work on ML + font.

Open research question: should we care about "dynamic typography"? One one hand it is an interesting research problem as typography has mainly been focusing on static fonts, on the other hand the application might be much narrower (readability and visual comfort might be more important for reading large chunks of static texts than a few dynamic fonts). (edited) 
}%liyi
}
\item[March 30, 2022]
{
\liyi{
One way to think about our project is to design a "semantic space" on top of "typography space" on top of "shape/animation space", in a 3-tier hierarchy from high to low levels, so that users can focus on the high level semantics (application/domain dependent emotion, object, speech, etc.), which in turn automatically drives the typography space which in turn drives the shape/animation space.

This hierarchical design is akin to \cite{Ma:2022:S3A} on layered authoring UI for stylized animations, but there, we only have 2 levels corresponding to the typography and animation spaces here.
We don't really need "semantics" for that project (aside from contact/collision), which would be more relevant for this one.
}%liyi
}
\item[March 18, 2022]
{
\liyi{
There are many great examples in \cite{Ma:2022:EKT:DE} and in the slack channel; one high level thing we can focus on is: which effects are better left for individual creativity and which can be automated to reduce tedious manual work?
}%liyi
}
\item[January 11, 2022]
{
\jiaju{
Hi @lwei @rhabib (tagging Rubaiat here so he can refer to this later), I have updated the paper draft with many more related works and a summary of my newest project idea (In the January 11 update).

Overall, I think we can propose a new type of stylized/animated texts called {\em Embodied Captions} that not only changes/animates its own appearance like kinetic typography but also interacts with the video content itself in some ways, like embodied performance on screen (like in the Body-Driven Graphics paper). We can draw from Embodied Cognition literature as well as works like Constructing Embodied Algebra by Sketching to inform and support our design decisions.

In terms of contributions, I think we can contribute 1) a design framework that guides the design and implementation of embodied captions, and 2) an authoring system that automatically adds embodied captions to live videos while allowing users to predefine/customize certain behaviors.
}%jiaju

\liyi{
Very comprehensive literature survey and amazing initial ideas! I have drafted paper title and abstract; feel free to take a look and comment/edit, based on which I can then submit a project proposal.
(We will need more brainstorming to refine the project idea and scope, but that can be for later.)
}%liyi
}
\item[January 11, 2022]
{
\jiaju{
\paragraph{Overall idea}
Below you can find a long list of related works I found recently that are highly relevant. From my recent search, I discoverd there have been a decent amount of work on stylizing captions/subtitles (I am going to use these two words interchangebly) to express non-verbal information like sound effects, music, tone, and, more commonly, emotions. These ``stylized'' captions adopt some forms of kinetic typography but are different from kinetic typography videos seen in~\cite{Kato:2015:TLI} in that the contents of kinetic typogrpahy videos are mainly focused on the animated texts themselves, while stylized captions are closer to closed captions that are added onto videos. For this reason, I think stylized captions are closer to our core project idea.

Works by Janine~\cite{Butler:2018:ICS,Butler:2018:ECM} proposed an interesting term called \textbf{``embodied captions.''} In a nutshell, this refers to designing animated captions that not only changes/animates its own appearance but also interacts with the video content itself in some ways (embodied performance on screen). ``Embodied captions'' ``embody the meaning of the video''~\cite{Butler:2018:ECM} and has a theory rooted in embodied cognition (a theory that centers around bodily movements can help us understand and perceive things), which was explored in the Constructing Embodied Algebra by Sketching paper by Saquib et al.~\cite{Saquib:2021:CEA}. In our work, we could build a system similar to the Body-Driven Graphics paper by Saquib et al.~\cite{Saquib:2019:IBD} that allows users to map hand and body gestures to animate captions.

Overall, despite the abundance of prior works, they mainly use stylized captions to express one or a few forms of information (expressing emotions~\cite{Lee:2007:EC}, displaying sound effects~\cite{Wang:2017:VVS}), are mainly focused on video post-processing (no live streaming use cases), lack a general design framework that guides the design of the appearance, animations, and interactions (with video contents) of embodied captions. I think in our work, we can contribute two things: 
\begin{enumerate}
    \item Firstly, we propose a general design framework that can help people more efficiently create embodied captions via post-processing. This framework should define how various attributes of captions (font, typography, color, text frames, animation (distortions, motions), placement on the screen, body interactions, etc) should be used to convey various information like speech, emotion, sound effects, etc. We can first extract a set of basic principles from prior work, and then refine it by interviewing professional and frequent live streaming audiences. I envision the structure of this to be similar to the Beyond Show of Hands paper by Chung et al.~\cite{Chung:2021:BSH}
    \item Secondly, we then create a system that adds embodied captions automatically to live videos based on our proposed design framework. Major parts of this system should be automated, since live streaming is mostly not prescripted. For example, to detect emotions, we could use Microsoft's Emotion API like in this paper~\cite{Liu:2018:RBE}, and we can use libraries like Google MediaPipe for motion and hand tracking. We should also allow users to predefine some subtitles by entering a text script and adding stylized effects with our tool. We should also provide them with some templates to start with (the templates could be part of the design framework we proposed).
\end{enumerate}
}%jiaju
}


==> note_2023.tex <==
\item[July 2, 2023: Use of Copyrighted Music Video Material in Accepted UIST Submission \#8580]
{Use of Copyrighted Music Video Material in Accepted UIST Submission \#8580
\jiaju{
Dear UIST 2023 Program Chairs,

My name is Jiaju Ma and I am the first author of the conditionally accepted UIST submission \#8580.
This work is about automatically adding lyric text to existing music videos, so in the paper we have screenshots of popular music videos with lyrics added (please refer to the attached figures).
These music videos are uploaded by the artists themselves officially (or the company they belong to) and are copyrighted (such as \href{https://youtu.be/pc_2ZKB4LVc}{this one}).
I wonder if we should somehow obtain licenses to use these screenshots?
Or does this fall under \href{https://www.acm.org/publications/authors/guidance-for-authors-on-fair-use}{Fair Use}?

Moreover, in the supplemental material, we have music videos with added lyrics to demonstrate the effectiveness of our proposed pipeline (an example video is also attached to this email).
The videos are excerpts of the original music videos and contain portions of the corresponding song.
I wonder if these require licenses as well.

The main concern here is that these videos belong to big companies and might charge a hefty fee even for non-commercial uses, and obtaining the needed licenses might take quite a while too.

Thanks so much for your time and help!

Sincerely,
Jiaju
}%jiaju
}
\item[March 20, 2023]
{
\jiaju{
 I think our main contributions should be 1) a set of design guidelines for lyric videos and 2) an automated pipeline that instantiate these guidelines, so I worked on a section called Design Guidelines.
 Can you take a look at that before our meeting on Tuesday?
 Feel free to leave comments here or directly in the paper draft
}%jiaju
}
\item[March 6, 2023]
{
\liyi{
One general approach for layout optimization is to combine preset templates and scene (image or video) content \cite{Yang:2016:AGV}, so that we can leverage both human expertise (e.g., having professional designers build the templates) and machine analysis (e.g., vide/image saliency).

\cite{Tang:2022:SS} proposes a system to place data visualization over videos. Despite the different applications (visualization versus animated text effects), the pipeline contains highly relevant design considerations and optimization methods.
For example, the 8 design considerations (see their Figure 3) include: (1) insert one data visualization for each shot, (2) use simple visualizations that are easy to follow, (3) color visualizations to keep in harmony with videos, (4) follow basic aesthetic principles when placing data visualizations, (5) place data visualizations next to the references, (6) place data visualizations in the spare space, (7) place data visualizations at consecutive shots in the same region, (8) elongate or shorten data shots to match music beats. By simply replacing “visualization” with “text” these can almost directly apply to our scenarios.
The layout optimization algorithm (their Figure 5) considers balance, alignment, proximity, readability, and coherence, all of which can be applied to animated text effects.

There are various detailed vision/ML method components that consider image/video content (e.g., saliency) to optimize for layout placement, such as:
\begin{itemize}
\item
\cite{Li:2022:HTL} optimizes text layout over images by (1) saliency analysis and (2) aesthetic layout evaluation. The latter might have implicitly taken into account background image contrast (need detailed checking) but in any case, there is a specific module deciding when and where to add a background mask to enhance text readability.

\item
\cite{Liang:2018:AGT} proposes a simple method to place (advertisement) labels over videos: (1) compute saliency of each video frame, including human face, (2) select among 4 areas (top, bottom, left, right) that has minimal saliency while also maintaining temporal coherence with a stability control parameter, (3) decide font size to fit into the selected area, (4) choose font color in harmony with the background region.

\item
\cite{Zhao:2017:AGV} proposed a simple face-aware text layout method to generate representative images from videos.
\end{itemize}

Note that scene-aware layout is different from general layout optimization for graphics design or webpages which can freely arrange input elements without being constrained by a background image/video.
}%liyi
}
\item[February 18, 2023]
{
\liyi{
Analogous to automatic visual generation from transcripts/captions/spoken-words \cite{Leake:2020:GAV,Liu:2023:VC}, we propose a system that automatically generates kinetic typography from music lyric videos, including the word timing and style (font, color, size, position, etc.).
The system should be able to provide good defaults for one-click authoring, while allowing users to customize more detailed effects (TBD).

The main technical contributions/challenges would include: analyze the lyrics (NLP), music (pitches and beats), and video content (background and foreground) to figure out the best way to place and render the texts, so that they are timed and moved and stylized as though done by professional producers/artists.

This is more of an umbrella direction and the scope might exceed a single publon, for which we can narrow down a bit.
}%liyi

\liyi{
Another less related direction is automatic video cutting from transcript, the sort of mixed initiative tools that Maneesh interested in.
}%liyi
}


==> old/table_variation.tex <==
\begin{table}[t]
    \small
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
    \textbf{Design Guidelines} & Var. A  & Var. B & Var. C & Var. D & Var. E \\\midrule
    \nothing{Lyric Flash Composition - }DG1\&2  & \cmark&\xmark& \cmark         &      \cmark     & \cmark         \\\hline
    \nothing{Text Presentation - }DG 3\&4       & \cmark& \cmark         &\xmark& \cmark         & \cmark         \\\hline
    \nothing{Text-Audio Coordination - }DG 5    & \cmark& \cmark         & \cmark         &\xmark& \cmark         \\\hline
    \nothing{Text-Video Coordination - }DG 6\&7 & \cmark& \cmark         & \cmark         & \cmark         &\xmark \\\bottomrule
    \end{tabular}
	}
    \Caption{Table showing how each ablated variation is constructed.}
    {%
    \liyi{(March 30, 2023) I recommend defining all these DGs inside \filename{symbols.tex} as well to help maintain cross-reference consistency when we add, delete, or reorder them in \Cref{sec:design}.}
    }
    \label{table:pipeline_ablation}
\end{table}

==> package.tex <==
\usepackage{color}
%\usepackage{epsfig}
%\usepackage{psfig}
%\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
\usepackage{ifthen}
%\usepackage[draft]{hyperref} % new acmsiggraph.cls
\usepackage{float}
\usepackage{alltt}
%\usepackage{mathenv}
\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage{rotating}
\usepackage{newlfont} % for Box
%\usepackage{ulem}
\usepackage{floatflt}
\usepackage{wrapfig}
\usepackage{fixltx2e}
\usepackage{subfig} % for subfloat
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{cleveref}
\usepackage{algorithmic}
%\usepackage{slashbox}
% \usepackage[export]{adjustbox}
\usepackage{mathtools, cuted}
\usepackage{CJKutf8} % Chinese
\usepackage{enumitem}% http://ctan.org/pkg/enumitem
% \usepackage{mmstyle}% add by Anyi for math term
\usepackage[ruled]{algorithm2e} % For algorithms
\usepackage{layouts}
\usepackage{pifont}% http://ctan.org/pkg/pifont


==> paper.tex <==

\input{package}
\input{macros}
\input{symbols}
\input{graphicspath}
\input{uist2023}

\begin{document}

\input{title_author}

\input{fig_teaser}

\input{copyright}

\input{abstract}

\input{ccs}

\maketitle

\input{introduction}
\input{prior}
% \input{background} % \liyi{background should be after prior and before design for better coherence}
\input{design}
% \input{interface}
\input{method}
\input{result}
\input{evaluation}
\input{limitations}
\input{conclusion}
\input{ack}

% \balance{}

\bibliographystyle{ACM-Reference-Format}
{
\bibliography{paper,misc}
}

\newpage %\liyi{(July 24, 2023) improve the layout a bit}
\appendix
\normalsize

\input{supp}

\ifthenelse{\equal{\final}{0}}
{
\clearpage
\pagenumbering{roman}

\input{note}
}
{}

\end{document}


==> symbols.tex <==
% institutions
\newcommand{\adobeResearch}{Adobe Research}
\newcommand{\stanford}{Stanford University}
\newcommand{\roblox}{Roblox}

% Einstein
\newcommand{\energy}{E}
\newcommand{\mass}{m}
\newcommand{\lightspeed}{c}

% dart throwing
\newcommand{\domainsym}{\Omega}
\newcommand{\dimnumber}{d} % dimensionality of the sample space
% note it should be $k$-d not $k$-$d$ as here "d" is an acronym for the word "dimension," not a variable.

\newcommand{\samplesym}{s}
\newcommand{\sample}{\samplesym{}}
\newcommand{\samplesetsym}{\mathcal{S}}
\newcommand{\sampleset}{\samplesetsym{}}
\newcommand{\sampleprime}{\samplesym^{\prime}{}}
\newcommand{\dist}{d}
\newcommand{\conflictdist}{r}
\newcommand{\union}{\oplus}
\newcommand{\failure}{f}
\newcommand{\assign}{\leftarrow}

\newcommand{\inputmv}{\mathcal{V}}
\newcommand{\shot}{s}
\newcommand{\lyricflash}{l}
\newcommand{\lyricPhrase}{l}
\newcommand{\textkernel}{k}
\newcommand{\wordthreshold}{\delta}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\dg}{\textbf{DG}}
\newcommand{\dgPhrase}{\textbf{\dg1}}
\newcommand{\dgLinebreak}{\textbf{\dg2}}
\newcommand{\dgHighlight}{\textbf{\dg3}}
\newcommand{\dgContrast}{\textbf{\dg4}}
\newcommand{\dgTiming}{\textbf{\dg5}}
\newcommand{\dgFocus}{\textbf{\dg6}}
\newcommand{\dgSpatial}{\textbf{\dg7}}

\newcommand{\energyPrev}{E_{\text{prv}}}
\newcommand{\energyContrast}{E_{\text{cnt}}}
\newcommand{\energyFocus}{E_{\text{att}}}
\newcommand{\energyVisualCenter}{E_{\text{fcs}}}
\newcommand{\energyOverlap}{E_{\text{fgd}}}

\newcommand{\spannedFrames}{\mathcal{F}}
\newcommand{\focusMask}{s_{\text{fcs}}}
\newcommand{\foregroundMask}{s_{\text{fgd}}}
\newcommand{\avgFocusMask}{\bar{s}_{\text{fcs}}}
\newcommand{\avgForegroundMask}{\bar{s}_{\text{fgd}}}

\newcommand{\resultsSite}{\url{https://hci.stanford.edu/research/lyricvideo/}}

==> title_author.tex <==

\title{Using Paper Drafts to Manage Research Projects}
\title{Kinetic Typography for Live Transcript Visualization} % \jiaju{(December 25, 2021) Temp title}

\title{Embodied Kinetic Typography} %\liyi{January 11, 2022) New title combining main aspects of the current idea, could be too short/terse but we can gradually refine.}

\title{A Text-based Authoring Tool for Augmenting Video Subtitles with Kinetic Typography} %\jiaju{May 19, 2022} New title based on current demo and potential exit talk title


\title{Creating Kinetic Video Captions via Direct Text Manipulation} % \liyi{(May 19, 2022) simplify/consolidate the title a bit}

\title{Designing Readable Lyric Videos} % \jiaju{March 20, 2023} \liyi{It is not just about readability, as there must be some other functional and artistic considerations?}

\title{Animating Stylized Lyric Texts for Music Videos} %\liyi{(March 20, 2023) See if this is better}

\title{Generating Readable Captions for Music Lyric Videos} % \liyi{(March 28, 2023) Rubaiat commented that the title above is misleading; see if this one is better}

\title{Generating Readable Subtitles for Music Lyric Videos} % \liyi{(March 29, 2023) After checking https://www.veed.io/learn/closed-captioning-vs-subtitles for caption versus subtitle I think we are right to stick to the latter.}

\title{Designing Readable and Focused Lyric Videos} %liyi{(March 30, 2023) what we mean by "focused"? Would "contextual" be a more accurate term (depending on exactly what you mean)? Also, it is not clear from this title which part we aim to be "readable".}

\title{Designing Legible Music Lyric Videos} % \liyi{(March 30, 2023) I am reading a book titled "a history of graphic design" from which "legible" seems a more standard term than "readable". Still, I don't think this title (changed from the one above) is specific enough with regard to exactly which part we want to be legible.}

\title{Generating Legible Subtitles for Music Lyric Videos} % \liyi{(March 30, 2023) IMHO this title best depicts this research, but feel free to add new variations below with comments about your reasoning.}

\title{Automated Conversion of Music Videos into Lyric Videos}


\author{Jiaju Ma}
\affiliation{
    \institution{\stanford}
    \country{}
}
\author{Anyi Rao}
\affiliation{
    \institution{\stanford}
    \country{}
}

\author{Li-Yi Wei}
\affiliation{
    \institution{\adobeResearch}
    \country{}
}

\author{Rubaiat Habib Kazi}
\affiliation{
    \institution{\adobeResearch}
    \country{}
}
\author{Valentina Shin}
\affiliation{
    \institution{\adobeResearch}
    \country{}
}

% \author{John Nelson}
% \affiliation{\institution{\adobeResearch}}

\author{Maneesh Agrawala}
\affiliation{
    \institution{\stanford}
    \country{}
}
\affiliation{
    \institution{\roblox}
    \country{}
}

==> tog.tex <==
\acmJournal{TOG}
\acmYear{2017}
\acmVolume{36}
\acmNumber{4}
\acmArticle{1}
\acmMonth{7} % July
\acmDOI{}
\acmSubmissionID{papers\_0001}



==> uist2023.tex <==
\copyrightyear{2023}
\acmYear{2023}
\acmConference[UIST '23]{The 36th Annual ACM Symposium on User Interface Software and Technology}{October 29-November 1, 2023}{San Francisco, CA, USA}
\acmBooktitle{The 36th Annual ACM Symposium on User Interface Software and Technology (UIST '23), October 29-November 1, 2023, San Francisco, CA, USA}
\acmPrice{15.00}
\acmDOI{10.1145/3586183.3606757}
\acmISBN{979-8-4007-0132-0/23/10}

